RITUAL: Random Image Transformations as a Universal Anti-hallucination Lever in Large Vision Language Models

Recent advancements in Large Vision Language Models (LVLMs) have revolutionized how machines understand and generate textual responses based on visual inputs, yet they often produce "hallucinatory" outputs that misinterpret visual information, posing challenges in reliability and trustworthiness. We propose RITUAL, a simple decoding method that reduces hallucinations by leveraging randomly transformed images as complementary inputs during decoding, adjusting the output probability distribution without additional training or external models. Our key insight is that random transformations expose the model to diverse visual perspectives, enabling it to correct misinterpretations that lead to hallucinations. Specifically, when a model hallucinates based on the original image, the transformed images -- altered in aspects such as orientation, scale, or color -- provide alternative viewpoints that help recalibrate the model's predictions. By integrating the probability distributions from both the original and transformed images, RITUAL effectively reduces hallucinations. To further improve reliability and address potential instability from arbitrary transformations, we introduce RITUAL+, an extension that selects image transformations based on self-feedback from the LVLM. Instead of applying transformations randomly, RITUAL+ uses the LVLM to evaluate and choose transformations that are most beneficial for reducing hallucinations in a given context. This self-adaptive approach mitigates the potential negative impact of certain transformations on specific tasks, ensuring more consistent performance across different scenarios. Experiments demonstrate that RITUAL and RITUAL+ significantly reduce hallucinations across several object hallucination benchmarks.

==> _rebuttal.tex <==
% \input{_constants}
% \rebuttal

% \documentclass[10pt,twocolumn,letterpaper]{article}
% \input{cvpr_header}
% \myexternaldocument{_main}
% \begin{document}
% %% TITLE
% \title{\paperTitle}
% \maketitle
% \thispagestyle{empty}
% \appendix
% %%

% We thank the reviewers for their comments.

% {\small
% \bibliographystyle{ieeenat_fullname}
% \bibliography{11_references}
% }

% \end{document}


==> figures/04llava_bench.tex <==
\begin{figure*}[t!]
    \centering
    % \vspace{-3mm}
    \includegraphics[width=\textwidth]{figures/llava_bench.pdf}
    \vspace{\abovefigcapmargin}
    % \vspace{-3mm}
    \caption{
    \textbf{Qualitative results on LLaVA-Bench~\citep{liu2023visual}.}
    Hallucinations are highlighted in {\color{red}{red}}.
    \Ours well understands ambiguous images and effectively mitigates hallucinations in outputs.
    % \jh{
    % Illustration of hallucination reduction by our proposed \Ours on LLaVA-Bench benchmark. Hallucinations are highlighted in \color{red}{red}.
    % }
    }%
    \label{fig:llava_bench}
    % \vspace{\belowfigcapmargin}
    \vspace{-4mm}
\end{figure*}

==> figures/06description_case.tex <==
\begin{figure*}[t!]
    \centering
    \vspace{-3mm}
    \includegraphics[width=0.9\textwidth]{figures/description_example.pdf}
    % \vspace{\abovefigcapmargin}
    \vspace{-3mm}
    \caption{
        \textbf{\Ours in descriptive task.}
        \Ours refines the probability distribution to generate the correct token during decoding, thereby mitigating hallucinations in the following generated text.
        \todo{fig1랑 합치기. fig1으로 이동}
    }%
    \label{fig:descriptive_task}
    \vspace{\belowfigcapmargin}
    % \vspace{-3mm}
\end{figure*}



% \begin{table*}[t!]

% \begin{minipage}[t!]{\textwidth}
%   \begin{minipage}[t!]{0.65\textwidth}
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/description_example.pdf}
%     \captionof{figure}{\textbf{\Ours on descriptive task.}}
%   \label{fig:descriptive_task}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.33\textwidth}
%     \vspace{-2cm}
%     \captionof{table}{
%         \textbf{Ablation of the number of augmented images in \Ours on COCO dataset.}
%       }
%     \centering
%     \scalebox{0.9}{
%     \begin{tabular}{ccc}
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\# of Aug.\\ Images\end{tabular}} & \multicolumn{2}{c}{LLaVA-1.5} \\ \cmidrule(lr){2-3}
%                   & Acc.  & F1    \\ \hline
% 1                 & 88.87 & 88.81 \\
% 2                 & \colorbox{SecondBest}{89.07} & \colorbox{SecondBest}{89.02} \\
% 3                 & \colorbox{Best}{89.17} & \colorbox{Best}{89.16} \\ 
%                     % \midrule

% % 1                 & \colorbox{SecondBest}{85.83} & \colorbox{SecondBest}{86.17} \\
% % 2                 & 85.37 & 85.69 \\
% % 3                 & \colorbox{Best}{86.20} & \colorbox{Best}{86.61} \\ \midrule

% % 1                 & 78.80 & 80.54 \\
% % 2                 & \colorbox{Best}{79.10} & \colorbox{Best}{80.87} \\
% % 3                 & \colorbox{SecondBest}{79.07} & \colorbox{SecondBest}{80.80} \\
% \bottomrule
% \end{tabular}

%     }
%     \label{tab:multiple augmentated images_main}
%     \end{minipage}
%   \end{minipage}
%    \vspace{-4mm} 
% \end{table*}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/04amber.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength\tabcolsep{3pt} % base value: 6pt
    \scalebox{0.96}{
    \begin{tabular}{llx{27}x{27}x{27}x{27}x{27}x{27}x{27}x{27}x{32}}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Generative}} & \multicolumn{4}{c}{\textbf{Discriminative}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\makecell{AMBER \\ Score}}}}\\
        \arrayrulecolor{gray} \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
         & & CHAIR & Cover & Hal & Cog & Acc. & Prec. & Rec. & F1 & \\
        \arrayrulecolor{gray} \midrule
        \multirow{4}{*}{\textbf{LLaVA 1.5~\citep{liu2024visual}}} & \textit{base} & 58.8 & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & VCD & 58.8 & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & M3ID & 58.8 & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & Ours & 58.8 & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
        \arrayrulecolor{gray} \midrule
        \multirow{4}{*}{\textbf{InstructBLIP~\citep{dai2024instructblip}}} & \textit{base} & 54.6 & 24.8 & 32.6 & 10.7 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & VCD & 58.8 & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & M3ID & \colorbox{SecondBest}{58.8} & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & Ours & \colorbox{Best}{58.8} & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
        \arrayrulecolor{gray} \midrule
        \multirow{4}{*}{\textbf{Qwen-VL~\citep{bai2023qwen}}} & \textit{base} & 54.6 & 24.8 & 32.6 & 10.7 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & VCD & 58.8 & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & M3ID & \colorbox{SecondBest}{58.8} & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
         & Ours & \colorbox{Best}{58.8} & 23.7 & 31.8 & 9.9 & 9.9 & 23.7 & 31.8 & 9.9 & 9.9 \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{\abovetabcapmargin}
    \caption{
        \textbf{Results on AMBER~\citep{wang2023llm} benchmark.}
        LLaVA 1.5~\citep{liu2024visual} InstructBLIP~\citep{dai2024instructblip}
        The \textit{base} denotes the standard decoding.
        outperform contrastive decoding baselines: VCD~\citep{leng2023mitigating} and M3ID~\citep{favero2024multi}.
    }
    \vspace{\belowtabcapmargin}
    \label{tab:AMBER}
\end{table*}

==> tables/11self_feedback.tex <==
% \begin{table*}[t!]
%     \centering
%     \small
%     \setlength{\tabcolsep}{5pt} % base value: 6pt
%     \scalebox{0.9}{
%     \begin{tabular}{cy{40}x{30}x{30}x{30}x{30}x{30}x{30}x{30}x{30}}
%     \toprule
%     \multirow{2}{*}{\textbf{MS-COCO~\citep{lin2014microsoft}}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{LLaVA 1.5~\citep{liu2023visual}}} & \multicolumn{4}{c}{\textbf{InstructBLIP~\citep{dai2024instructblip}}} \\
%     \arrayrulecolor{gray} \cmidrule(lr){3-6} \cmidrule(lr){7-10}
%     &  & {{Acc.} {\up}} & {{Prec.} {\up}} & {{Rec.} {\up}} & {{F1} {\up}} & {{Acc.} {\up}} & {{Prec.} {\up}} & {{Rec.} {\up}} & {{F1} {\up}} \\
%     \midrule
%     \multirow{3}{*}{\textbf{Random}} & \textit{base} & 84.13 & 82.86 & 86.07 & 84.43 & 82.80 & 82.24 & 83.67 & 82.95 \\
%     & \textbf{\Ours} & \colorbox{SecondBest}{88.87}	& \colorbox{Best}{89.23} & \colorbox{SecondBest}{88.40} & \colorbox{SecondBest}{88.81} & \colorbox{Best}{88.83} & \colorbox{Best}{90.48} & \colorbox{Best}{86.80} & \colorbox{Best}{88.60} \\
%     & \textbf{\Oursplus} & \colorbox{Best}{89.17}	& \colorbox{SecondBest}{88.89} & \colorbox{Best}{89.53} & \colorbox{Best}{89.21} & {} & {} & {} & {} \\
%     \midrule
%     \multirow{3}{*}{\textbf{Popular}} & \textit{base} & 80.87 &	78.23 &	85.53 &	81.72 & 75.80	& 72.74 &	82.53 &	77.33 \\
%     & \textbf{\Ours} & \colorbox{Best}{85.83} & \colorbox{Best}{84.17} & \colorbox{SecondBest}{88.27} & \colorbox{Best}{86.17} & \colorbox{Best}{81.97} & \colorbox{Best}{78.90} & \colorbox{Best}{87.27} & \colorbox{Best}{82.87} \\
%     & \textbf{\Oursplus} & \colorbox{SecondBest}{85.40}	& \colorbox{SecondBest}{83.27} & \colorbox{Best}{88.60} & \colorbox{SecondBest}{85.85} & {} & {} & {} & {} \\
%     \midrule
%     \multirow{3}{*}{\textbf{Adversarial}} & \textit{base} & 76.23 & 71.75 & 86.53 & 78.45 & 75.40 & 71.60 & 84.20 & 77.39 \\
%     & \textbf{\Ours} & \colorbox{SecondBest}{78.80} & \colorbox{SecondBest}{74.43} & \colorbox{SecondBest}{87.73} & \colorbox{SecondBest}{80.54} & \colorbox{Best}{78.73} & \colorbox{Best}{74.57} & \colorbox{Best}{87.20} & {80.39} \\
%     & \textbf{\Oursplus} & \colorbox{Best}{79.17}	& \colorbox{Best}{74.48} & \colorbox{Best}{88.73} & \colorbox{Best}{80.99} & {} & {} & {} & {} \\
%     \bottomrule
%     \end{tabular}
%     }
%     % \vspace{\abovetabcapmargin}
%     \caption{
%         \textbf{Comparison of transformation selection.} \Ours (random selection) vs \Oursplus(self-feedback).
%     }
%     % \vspace{\belowtabcapmargin}
%     \label{tab:self_feedback}
% \end{table*}



\begin{table*}[t!]
    \caption{
        \textbf{Effect of self-feedback on transformation selection.} While, \Ours randomly selects image transformations, \Oursplus selects image transformation via self-feedback from LVLMs.
    \todo{remove}
    }
    \centering
    \small
    \setlength{\tabcolsep}{5pt} % base value: 6pt
    \scalebox{0.9}{
    \begin{tabular}{cy{40}x{30}x{30}x{30}x{30}}
    \toprule
    \multirow{2}{*}{\textbf{MS-COCO~\citep{lin2014microsoft}}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{LLaVA 1.5~\citep{liu2023visual}}} \\
    \arrayrulecolor{gray} \cmidrule(lr){3-6}
    &  & {{Acc.} {\up}} & {{Prec.} {\up}} & {{Rec.} {\up}} & {{F1} {\up}}\\
    \midrule
    \multirow{3}{*}{\textbf{Random}} & \textit{base} & 84.13 & 82.86 & 86.07 & 84.43 \\
    & \textbf{\Ours} & \colorbox{SecondBest}{88.87}	& \colorbox{Best}{89.23} & \colorbox{SecondBest}{88.40} & \colorbox{SecondBest}{88.81} \\
    & \textbf{\Oursplus} & \colorbox{Best}{89.17}	& \colorbox{SecondBest}{88.89} & \colorbox{Best}{89.53} & \colorbox{Best}{89.21} \\
    \midrule
    \multirow{3}{*}{\textbf{Popular}} & \textit{base} & 80.87 &	78.23 &	85.53 &	81.72  \\
    & \textbf{\Ours} & \colorbox{Best}{85.83} & \colorbox{Best}{84.17} & \colorbox{SecondBest}{88.27} & \colorbox{Best}{86.17} \\
    & \textbf{\Oursplus} & \colorbox{SecondBest}{85.40}	& \colorbox{SecondBest}{83.27} & \colorbox{Best}{88.60} & \colorbox{SecondBest}{85.85} \\
    \midrule
    \multirow{3}{*}{\textbf{Adversarial}} & \textit{base} & 76.23 & 71.75 & 86.53 & 78.45 \\
    & \textbf{\Ours} & \colorbox{SecondBest}{78.80} & \colorbox{SecondBest}{74.43} & \colorbox{SecondBest}{87.73} & \colorbox{SecondBest}{80.54} \\
    & \textbf{\Oursplus} & \colorbox{Best}{79.17}	& \colorbox{Best}{74.48} & \colorbox{Best}{88.73} & \colorbox{Best}{80.99} \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{\abovetabcapmargin}
    
    % \jh{LLaVA만 남기고 수정완}
    % \sm{굿}
    % }
    % \vspace{\belowtabcapmargin}
    \label{tab:self_feedback}
\end{table*}

==> tables/15mplug_larger.tex <==
\begin{table}[ht!]
\caption{\textbf{Results of mPLUG-owl2~\citep{ye2024mplug} on POPE benchmark.}
\todo{remove}}
\centering
\resizebox{.8\columnwidth}{!}{
\begin{tabular}{cllcccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Setup}       & \multirow{2}{*}{Method} & \multicolumn{4}{c}{mPLUG-owl2}                                    \\ \cmidrule(lr){4-7}
                         &                              &                         & Acc.           & Prec.          & Rec.           & F1             \\ \hline


\multirow{18}{*}{COCO} & \multirow{5}{*}{Random}                       & \textit{base}                & 81.00          & 75.27          & \colorbox{Best}{92.33} & 82.93          \\
                         &                              & VCD                     & \colorbox{SecondBest}{81.53}    & \colorbox{SecondBest}{76.40}    & 91.27          & \colorbox{SecondBest}{83.17}          \\
                         &                              & M3ID                    & 80.90          & 75.29          & 92.00          & 82.81    \\
                         &                              & DoLa                    & 81.20 & 75.97 & 91.27 & 82.92    \\
                         &                              & \Ours                  & \colorbox{Best}{84.83} & \colorbox{Best}{80.40} & \colorbox{SecondBest}{92.13}    & \colorbox{Best}{85.87} \\ 
                         
                         
                         \cmidrule(lr){2-7}

                         
                         & \multirow{5}{*}{Popular}     & \textit{base}                & 76.27          & 69.96          & \colorbox{SecondBest}{92.07}    & 79.50    \\
                         &                              & VCD                     & 75.70          & 69.88          & 90.33          & 78.80          \\
                         &                              & M3ID                    & 76.50          & 70.23          & 92.00          & 79.65          \\

                         &                              & DoLa                    & \colorbox{SecondBest}{76.67}    & \colorbox{SecondBest}{70.58}    & 91.47          & \colorbox{SecondBest}{79.67}    \\
                         
                         &                              & \Ours                  & \colorbox{Best}{80.43} & \colorbox{Best}{74.64} & \colorbox{Best}{92.20} & \colorbox{Best}{82.49} \\ 
                         
                         \cmidrule(lr){2-7}

                         
                         & \multirow{5}{*}{Adversarial} & \textit{base}                & 73.20          & 66.88          & \colorbox{SecondBest}{91.93}    & \colorbox{SecondBest}{77.43}          \\
                         &                              & VCD                     & \colorbox{SecondBest}{73.23}    & \colorbox{SecondBest}{67.26}    & 90.53          & 77.18 \\
                         &                              & M3ID                    & 72.57          & 66.28          & 91.87          & 77.00          \\

                         & & DoLa                    & 72.37          & 66.29          & 91.00          & 76.71    \\

                         
                         &                              & \Ours                  & \colorbox{Best}{75.23} & \colorbox{Best}{68.88} & \colorbox{Best}{92.07} & \colorbox{Best}{78.80}    \\ \hline


                         
\multirow{17}{*}{A-OKVQA} & \multirow{5}{*}{Random}                       & \textit{base}                & 78.13          & \colorbox{SecondBest}{70.87}    & 95.53          & 81.37          \\
                         &                              & VCD                     & 77.70          & 70.42          & 95.53          & 81.07          \\
                         &                              & M3ID                    & \colorbox{SecondBest}{78.23}    & 70.73          & \colorbox{Best}{96.33} & \colorbox{SecondBest}{81.57}    \\
                         & & DoLa                    & 77.67 & 70.38 & 95.53 & 81.05    \\
                         
                         &                              & \Ours                  & \colorbox{Best}{80.20} & \colorbox{Best}{73.02} & \colorbox{SecondBest}{95.80}    & \colorbox{Best}{82.87} \\ 
                         
                         \cmidrule(lr){2-7}

                         
                         & \multirow{5}{*}{Popular}     & \textit{base}                & \colorbox{SecondBest}{71.27}    & \colorbox{SecondBest}{64.43}    & 94.93          & \colorbox{SecondBest}{76.77}    \\
                         &                              & VCD                     & 71.07          & 64.21          & 95.20          & 76.69          \\
                         &                              & M3ID                    & 69.57          & 62.80          & \colorbox{Best}{96.00} & 75.93          \\

                         & & DoLa                    & 71.10 & 64.22 & 95.27 & 76.72    \\
                         
                         &                              & \Ours                  & \colorbox{Best}{74.20} & \colorbox{Best}{66.96} & \colorbox{SecondBest}{95.53}    & \colorbox{Best}{78.74} \\ 
                         
                         \cmidrule(lr){2-7}

                         
                         & \multirow{4}{*}{Adversarial} & \textit{base}                & 64.83          & 59.15          & \colorbox{SecondBest}{95.87}    & 73.16          \\
                         &                              & VCD                     & \colorbox{Best}{66.43} & \colorbox{Best}{60.39} & 95.53          & \colorbox{Best}{74.00} \\
                         &                              & M3ID                    & 65.13          & 59.33          & \colorbox{Best}{96.27} & 73.41          \\

                         & & DoLa                    & 65.73 & 59.91 & 95.13 & 73.52    \\

                         
                         &                              & \Ours                  & \colorbox{SecondBest}{65.93}    & \colorbox{SecondBest}{59.99}    & 95.67          & \colorbox{SecondBest}{73.74}    \\ \hline
                         
\multirow{17}{*}{GQA}    & \multirow{5}{*}{Random}      & \textit{base}                & 80.00          & 74.04          & 92.40          & 82.21          \\
                         &                              & VCD                     & \colorbox{SecondBest}{81.60}          & \colorbox{Best}{77.56} & 88.93          & 82.86          \\
                         &                              & M3ID                    & 80.93          & 74.95          & \colorbox{SecondBest}{92.93}    & \colorbox{SecondBest}{82.98}    \\

                         & & DoLa                    & 78.67 & 73.19 & 90.47 & 80.92    \\

                         
                         &                              & \Ours                  & \colorbox{Best}{82.10} & \colorbox{SecondBest}{76.10}    & \colorbox{Best}{93.60} & \colorbox{Best}{83.95} \\ 
                         
                         \cmidrule(lr){2-7}

                         
                         & \multirow{5}{*}{Popular}     & \textit{base}                & \colorbox{SecondBest}{71.53}    & 64.94          & \colorbox{SecondBest}{93.60}    & \colorbox{SecondBest}{76.68}    \\
                         &                              & VCD                     & 71.40          & \colorbox{SecondBest}{65.77}    & 89.27          & 75.74          \\
                         &                              & M3ID                    & 71.50          & 65.06          & 92.87          & 76.52          \\

                         & & DoLa                    & 71.03 & 65.23 & 90.07 & 75.67    \\

                         
                         &                              & \Ours                  & \colorbox{Best}{73.47} & \colorbox{Best}{66.60} & \colorbox{Best}{94.13} & \colorbox{Best}{78.01} \\ 
                         
                         \cmidrule(lr){2-7}
                         
                         & \multirow{5}{*}{Adversarial} & \textit{base}                & 68.73    & 62.60    & \colorbox{SecondBest}{93.07}    & 74.85    \\
                         &                              & VCD                     & \colorbox{Best}{71.67} & \colorbox{Best}{65.98} & 89.47          & \colorbox{Best}{75.95} \\
                         &                              & M3ID                    & 68.23          & 62.29          & 92.40          & 74.42          \\

                         & & DoLa                    & \colorbox{SecondBest}{69.50} & \colorbox{SecondBest}{63.51} & 91.67 & \colorbox{SecondBest}{75.03}    \\
                         
                         &                              & \Ours                  & 68.30          & 62.15          & \colorbox{Best}{93.60} & 74.70          \\ \bottomrule
\end{tabular}
}
\label{tab:mplug}
% \vspace{-0.05cm}
% \vspace{-0.1cm}
\end{table}
